Investigating the Impact of Choice on Deep Reinforcement Learning for Space Controls

For many space applications, traditional control methods are often used during operation. However, as the number of space assets continues to grow, autonomous operation can enable rapid development of control methods for different space related tasks. One method of developing autonomous control is Reinforcement Learning (RL), which has become increasingly popular after demonstrating promising performance and success across many complex tasks. While it is common for RL agents to learn bounded continuous control values, this may not be realistic or practical for many space tasks that traditionally prefer an on/off approach for control. This paper analyzes using discrete action spaces, where the agent must choose from a predefined list of actions. The experiments explore how the number of choices provided to the agents affects their measured performance during and after training. This analysis is conducted for an inspection task, where the agent must circumnavigate an object to inspect points on its surface, and a docking task, where the agent must move into proximity of another spacecraft and "dock" with a low relative speed. A common objective of both tasks, and most space tasks in general, is to minimize fuel usage, which motivates the agent to regularly choose an action that uses no fuel. Our results show that a limited number of discrete choices leads to optimal performance for the inspection task, while continuous control leads to optimal performance for the docking task.

==> old_intro_and_discussion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Intro
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Autonomous spacecraft operation is critical as the number of space assets grows and operations become more complex. For \textit{On-orbit Servicing, Assembly, and Manufacturing} (OSAM) missions, tasks such as inspection and docking enable the ability to assess, plan for, and execute different objectives. While these tasks may traditionally be accomplished using classical control methods, this requires constant monitoring and adjustment by human operators, which becomes challenging or even impossible as the complexity of the task increases. To this end, the importance of developing high-performing autonomy is growing.

\textit{Reinforcement Learning} (RL) is a fast-growing field with growing impact, spurred by success in agents that learn to beat human experts in games like Go \cite{silver2016mastering} and Starcraft \cite{starcraft2019}. RL is a promising application to spacecraft operations due to its ability to react in real-time to changing mission objectives and environment uncertainty \cite{ravaioli2022safe, hamilton2022zero}. However, in order for RL solutions to be used in the real world, they must control the spacecraft in a way that is acceptable to human operators.

In RL, it is common for agents to operate in a continuous control space at a specified frequency, where control values can be any value within a certain range. For space applications, where the agent controls the spacecraft's thrusters, this type of control may be inefficient, undesirable, or even impossible. Instead, it is often better for the spacecraft to choose from a discrete set of actions, where the thrusters are either fully on or off. In general, this follows Pontryagin's maximum principle \cite{kopp1962pontryagin}, which minimizes a cost function to find an optimal trajectory from one state to another. In this case, the cost is fuel use. In this paper, we compare RL agents trained using continuous control and this classical control principal to determine their advantages.

In this paper, we focus on two spacecraft tasks: \textit{inspection} (viewing the surface of another vehicle) and \textit{docking} (approach and joining with another vehicle). RL approaches have been used to solve many similar spacecraft inspection problems, including using RL to develop waypoints for an inspection mission \cite{LeiGNC22, AurandGNC23} and inspecting an uncooperative space object \cite{Brandonisio2021}. RL has also been used for similar docking problems, including a six degree-of-freedom docking task \cite{oestreich2021autonomous}, avoiding collisions during docking \cite{broida2019spacecraft}, and guidance for docking \cite{hovell2021deep}. This paper builds on previous work done to use RL to solve the inspection task with illumination \cite{vanWijkAAS_23} and the docking task \cite{ravaioli2022safe}. For the same docking task, the effect of Run Time Assurance during RL training was analyzed \cite{Dunlap2023, hamilton2023ablation}. For a 2D version of the docking task, LQR control was compared to a bang-bang controller \cite{dunlap2022hybrid}, similar to the agent with three discrete choices that will be analyzed in this paper.  

The main contributions of this work include answering the following questions.

% \todo{Restructure: I'm thinking (1) Does the RL agent need to easily be able to choose not to thrust? (2) At what point does adding more choices for the RL agent reduce performance? (3) Does the RL agent need finer granularity or choices with smaller magnitudes as the operating range changes?}

\begin{question}
\label{question:no-op}
    % Do we need to make no-op easier to choose?
    \Copy{q_text:no-op}{
    Does the RL agent need to easily be able to choose not to thrust?}
\end{question}
The most effective method to minimize fuel use is for the agent to choose not to thrust. As the number of choices increases, it becomes more difficult for the agent to choose a single value representing zero thrust. As the action magnitude decreases, it is also easier for the agent to choose actions that are closer to zero.

% \todo{Do you think decreasing $\controlmax$ also makes it easier to choose 0 or at least closer to 0? I would think it does but I don't know how to write up the justification}


\begin{question}
\label{question:granularity}
    % How does the task impact this? Do we need finer granularity or smaller magnitude as we get closer (i.e. reduce operating range)?
    \Copy{q_text:granularity}{
    Does the RL agent need finer granularity or choices with smaller magnitudes as the operating range changes?}
\end{question}
% \nph{Do we see different trends in choice numbers to performance depending on the task}
As the number of choices increases for these experiments, the granularity becomes finer. Additionally, two different action magnitudes are considered for each experiment. As the operating range changes from the inspection task to the docking task, the agent's performance based on these values will be analyzed.


\begin{question}
\label{question:num_choices}
    % How many choices is too many for an RL agent? reword At what point does adding more choices reduce performance? Does more choice make harder?
    \Copy{q_text:num_choices}{
    % At what point does adding more choices for the RL agent reduce performance?}
    Is there an optimal balance between discrete and continuous actions?}
\end{question}
% \todo{we should rethink the phrasing of this question because of the split answer. Focus more on something like "is there an optimal balance between discrete and continuous?" sort of thing. I don't think that phrasing is it, but I'll keep thinking on it.}
% \nph{can we get a discrete version to out-perform continuous for docking, or is it just pick discrete or continuous}
The number of choices will be varied over many different experiments, where continuous control gives the agent infinite choices. We will determine how many choices becomes too many for the agent, where performance starts to decrease.

\begin{quote}
    1. When a coarse discretization is used, the control output is not smooth, resulting in a
poor performance.
2. When a fine discretization is used, the number of states and the number of iteration steps become huge, which necessitates not only large memory storage but also many learning trials.
3. In order to keep the number of states manageable, an elaborate partitioning of the variables has to be found using prior knowledge.
\end{quote} \cite{doya2000reinforcement}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Discussion
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Discussion}
In this section, we answer the questions posed in the introduction by analyzing the overarching trends found in our experiments. In the interest of being concise, we include select results that highlight the trends we found and provide all the results in the Appendix.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Easy No-Op -> less deltaV?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\Paste{q_text:no-op}}
\noindent \textbf{Answer:} Yes. Increasing the likelihood of selecting ``no thrust" as an action greatly reduces $\deltav$ use.

\subsubsection{Discrete Action Space}

For agents with a discrete action space, having less choices means that it is easier for the agent to choose zero thrust. For the agent with three discrete choices, there is a $1$ in $3^3$ chance that the agent does not thrust at all, while for the agent with $101$ discrete choices, there is a $1$ in $101^3$ chance that the agent does not thrust at all. However, although it is harder for the agent to choose zero thrust with more choices, it enables the agent to choose actions with thrust closer to zero.

\figref{fig:delta-v-1.0-int-est} compares the $\deltav$ used by the final policies for each experiment with $\controlmax=1.0~N$. For the docking environment, it is clear that more choices leads to higher $\deltav$ use. This is also generally true for the inspection environment, but we see that 9, 11, and 21 choices lead to slightly lower $\deltav$ use. This occurs because the agents are able to choose actions that are close to zero, but not exactly zero, which helps the agents complete the task more efficiently.

\begin{figure}[ht]
\centering
\subfigure[Inspection environment.]{\includegraphics[width=\linewidth]{figures/inspection/1_0/DeltaV_int_est.png}\label{subfig:delta-v-1.0-insp}}\\
\subfigure[Docking environment.]{\includegraphics[width=\linewidth]{figures/docking/1_0/DeltaV_int_est.png}\label{subfig:delta-v-1.0-dock}}
\caption{Comparison of $\deltav$ ($~m/s$) for the final policies with $\controlmax=1.0~N$. Each marker represents the IQM of 100 trials, and the shaded region is the $95\%$ confidence interval about the IQM.}
\label{fig:delta-v-1.0-int-est}
\end{figure}

\figref{fig:delta-v-0.1-int-est} compares the $\deltav$ for the final policies with $\controlmax=0.1~N$. By reducing $\controlmax$, this makes it easier for the agent to choose actions that are closer to zero. For both environments, the agents trained with three discrete actions result in the lowest $\deltav$ use, but all other configurations result in similar $\deltav$ use.

\begin{figure}[ht]
\centering
\subfigure[Inspection environment.]{\includegraphics[width=\linewidth]{figures/inspection/0_1/DeltaV_int_est.png}\label{subfig:delta-v-0.1-insp}}\\
\subfigure[Docking environment.]{\includegraphics[width=\linewidth]{figures/docking/0_1/DeltaV_int_est.png}\label{subfig:delta-v-0.1-dock}}
\caption{Comparison of $\deltav$ ($~m/s$) for the final policies with $\controlmax=0.1~N$. Each marker represents the IQM of 100 trials, and the shaded region is the $95\%$ confidence interval about the IQM.}
\label{fig:delta-v-0.1-int-est}
\end{figure}

\subsubsection{Continuous Action Space}

For agents with a continuous action space, it is very difficult to choose zero thrust. For the inspection environment, \figref{fig:delta-v-1.0-int-est} shows that the agent with continuous actions uses almost as much $\deltav$ as the agent trained with 101 discrete actions. Therefore, to reduce $\deltav$ use, it is best to make it easier for the agent to choose actions closer to zero. This can be accomplished by reducing $\controlmax$.

\tabref{tab:con_insp} and \tabref{tab:con_dock} show the performance of the final policies with continuous actions across all metrics for the inspection and docking environments respectively. \tabref{tab:con_insp} shows that as $\controlmax$ is decreased from $1.0~N$ to $0.1~N$, the total reward, inspected points, and success rate all increase while $\deltav$ decreases. \tabref{tab:con_dock} similarly shows that as $\controlmax$ is decreased, the total reward and success rate increase while $\deltav$ decreases. Both cases show that allowing the agent to choose actions that are closer to zero enables better performance.


\begin{table*}[htb]
\centering
\caption{Inspection With Continuous Actions, IQM $\pm$ STD}
\begin{tabular}{llllll}
\toprule
$\controlmax$ & Total Reward & Inspected Points & Success Rate & $\deltav$ (m/s) & Episode Length (steps) \\
\midrule
$1.0~N$ & 7.8198 $\pm$ 0.5292 & 95.81 $\pm$ 4.6808 & 0.448 $\pm$ 0.4973 & 13.0222 $\pm$ 2.0929 & 323.98 $\pm$ 36.636 \\
$0.1~N$ & 8.7324 $\pm$ 0.199 & 99.0 $\pm$ 0.0 & 1.0 $\pm$ 0.0 & 10.8143 $\pm$ 1.7896 & 333.496 $\pm$ 13.6857 \\
\bottomrule
\end{tabular}
\label{tab:con_insp}
\end{table*}

\begin{table*}[htb]
\centering
\caption{Docking With Continuous Actions, IQM $\pm$ STD}
\begin{tabular}{lllllll}
\toprule
$\controlmax$ & Total Reward & Success Rate & $\deltav$ (m/s) & Violation (\%) & Final Speed (m/s) & Episode Length (steps) \\
\midrule
$1.0~N$ & 1.4105 $\pm$ 0.5279 & 0.57 $\pm$ 0.4951 & 13.2319 $\pm$ 1.7153 & 0.0 $\pm$ 0.0 & 0.0141 $\pm$ 0.0043 & 1780.944 $\pm$ 237.6564 \\
$0.1~N$ & 1.8289 $\pm$ 0.5193 & 0.842 $\pm$ 0.3647 & 11.6234 $\pm$ 1.3619 & 0.0 $\pm$ 0.0 & 0.0131 $\pm$ 0.0074 & 1497.154 $\pm$ 343.938 \\
\bottomrule
\end{tabular}
\label{tab:con_dock}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% More Granular = Better Performance?
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\Paste{q_text:granularity}}
\noindent \textbf{Answer:} It depends on the task. For the inspection task, action magnitude is more important. For the docking task, granularity is more important.

To answer this question, we first analyze what actions the agents take most often. \figref{fig:histogram} shows the percentage that each action is taken for the different experiments. For the inspection environment with $\controlmax=1.0~N$, close to 100\% of all actions taken are zero or very close to zero. However when $\controlmax=0.1~N$, the agents often choose actions that are either zero or $\pm \controlmax$. For the docking environment with $\controlmax=1.0~N$, while many actions taken are close to zero, there is a clear bell curve that appears centered on zero control. When $\controlmax=0.1~N$, this bell curve becomes more apparent, but the agents still tend to choose actions that are close to zero. These results suggest that action magnitude is more important in solving the inspection task, while granularity is more important in solving the docking task.

\begin{figure*}[ht]
\centering
\subfigure[Inspection environment with $\controlmax=1.0~N$]{\includegraphics[width=.32\linewidth]{figures/inspection/1_0/combined_action_histogram.png}}
\subfigure[Inspection environment with $\controlmax=0.1~N$]{\includegraphics[width=.32\linewidth]{figures/inspection/0_1/combined_action_histogram.png}\label{subfig:histogram-w}}
\subfigure[Docking environment with $\controlmax=1.0~N$]{\includegraphics[width=.32\linewidth]{figures/docking/1_0/combined_action_histogram.png}}
\subfigure[Docking environment with $\controlmax=0.1~N$]{\includegraphics[width=.32\linewidth]{figures/docking/0_1/combined_action_histogram.png}\label{subfig:histogram-bell}}
\subfigure{\includegraphics[width=.32\linewidth]{figures/inspection/0_1/histogram_legend.png}}
\caption{Comparison of actions taken in each environment. Each histogram shows the percentage of actions used the experiments, with the policies trained with continuous actions divided into 101 discrete intervals for comparison.}
\label{fig:histogram}
\end{figure*}


\subsubsection{Inspection}

For the inspection task, the total reward and inspected points for the final policies for each configuration is shown in \figref{fig:insp-reward-int-est}. The total reward represents the agent's ability to balance the objectives of inspecting all points and reducing $\deltav$ use. For the agents trained with $\controlmax=1.0~N$, it can be seen that all agents trained with 41 or less choices result in similar final reward. Recall that in \figref{subfig:delta-v-1.0-insp}, it can be seen that the lowest $\deltav$ for the inspection environment with $\controlmax=1.0~N$ occurs for the agent trained with 21 discrete actions. Notably, this is the configuration with the least number of choices where the agent can choose $u=0.1~N$.

For the agents trained with $\controlmax=0.1~N$, it can be seen that reward and number of inspected points tends to decrease as the number of choices increases. The agent trained with three choices results in the highest reward and inspected points, and \figref{subfig:delta-v-0.1-insp} shows that this configuration also results in the lowest $\deltav$ use. These results show that using a smaller action magnitude is much more important than increasing the granularity of choices for the inspection task. This result is intuitive as the agent does not need to make precise adjustments to its trajectory to complete the task, and can rely on following a general path to orbit the chief and inspect all points.

\begin{figure*}[ht]
\centering
\subfigure[Total reward with $\controlmax=1.0~N$]{\includegraphics[width=.48\linewidth]{figures/inspection/1_0/TotalReward_int_est.png}}
\subfigure[Total reward with $\controlmax=0.1~N$]{\includegraphics[width=.48\linewidth]{figures/inspection/0_1/TotalReward_int_est.png}}
\subfigure[Inspected points with $\controlmax=1.0~N$]{\includegraphics[width=.48\linewidth]{figures/inspection/1_0/InspectedPoints_int_est.png}}
\subfigure[Inspected points with $\controlmax=0.1~N$]{\includegraphics[width=.48\linewidth]{figures/inspection/0_1/InspectedPoints_int_est.png}}
\caption{Comparison of metrics for the final policies in the inspection environment. Each marker represents the IQM of 100 trials, and the shaded region is the $95\%$ confidence interval about the IQM.}
\label{fig:insp-reward-int-est}
\end{figure*}

\subsubsection{Docking}

For the docking task, the total reward and success rate for the final policies for each configuration is shown in \figref{fig:dock-reward-int-est}, where total reward represents the ability of the agent to balance successfully completing the task and minimizing $\deltav$ use. For the agents trained with $\controlmax=1.0~N$, the agents with more choices have the highest rewards and success rates. For the agents trained with $\controlmax=0.1~N$, outside of the agents with 3 and 51 choices, all other configurations result in similar rewards and success rates. Along with \figref{subfig:delta-v-1.0-dock} and \figref{subfig:delta-v-0.1-dock}, this shows that more choice and finer granularity leads to higher $\deltav$ use, but it is necessary to successfully complete the task.

However, there is one notable exception to this trend: the agents trained with continuous actions (highest granularity). It can be seen that this configuration uses by far the least $\deltav$ out of all agents that achieved at least a 50\% success rate. In particular, the agent trained with continuous actions and $\controlmax=0.1~N$ achieves the best balance of high reward and success with low $\deltav$. These results show that increasing the granularity of choices is much more important than using a smaller action magnitude for the docking task. This result is intuitive because the agent must be able to make precise adjustments to its trajectory as it approaches and docks with the chief.

\begin{figure*}[ht]
\centering
\subfigure[Total reward with $\controlmax=1.0N$]{\includegraphics[width=.48\linewidth]{figures/docking/1_0/TotalReward_int_est.png}}
\subfigure[Total reward with $\controlmax=0.1N$]{\includegraphics[width=.48\linewidth]{figures/docking/0_1/TotalReward_int_est.png}}
\subfigure[Success rate with $\controlmax=1.0N$]{\includegraphics[width=.48\linewidth]{figures/docking/1_0/Success_int_est.png}}
\subfigure[Success rate with $\controlmax=0.1N$]{\includegraphics[width=.48\linewidth]{figures/docking/0_1/Success_int_est.png}}
\caption{Comparison of metrics for the final policies in the docking environment. Each marker represents the IQM of 100 trials, and the shaded region is the $95\%$ confidence interval about the IQM.}
\label{fig:dock-reward-int-est}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Sweet sweet balance
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{\Paste{q_text:num_choices}}\label{sec:q-num_choices}
\noindent \textbf{Answer:} No, for these tasks it is better to choose either discrete or continuous actions.

% \todo{tie in value of looking at observed behavior to identify crucial actions and refine decisions on action space: see docking 1-0.1}
% \nph{I love the direction this is going and we should include the newest attempt at blending discrete and continuous. Have the best discrete results, continuous, and our attempts to beat it. That will show how we tried to find an optimal balance and the result is really just to pick one once you've identified what optimal should be like (bell vs W).}


To answer this question, we consider the behavior of the trained agents. \figref{fig:inspection_ep_plots_1} shows example trajectories of trained agents in the inspection task. Ideally, these agents will circumnavigate the chief along a smooth trajectory. In \figref{subfig:insp-ep-plot-con_1.0}, it can be seen that this is easily accomplished when the agent uses continuous actions, as it can constantly make small refinements to the trajectory to keep it smooth. On the other hand, when the agent can only use three discrete actions with $\controlmax=1.0~N$ as shown in \figref{subfig:insp-ep-plot-dis_1.0_3}, the trajectory becomes far less smooth. It can be seen that the agent jerks back and forth as it attempts to adjust its trajectory.

To balance continuous and discrete actions, the number of discrete choices can be increased to allow the agent make smaller adjustments to its trajectory. As seen in \figref{subfig:insp-ep-plot-dis_1.0_101}, having 101 choices helps the agent's trajectory become much smoother. However, as answered by question \qref{question:granularity}, this comes at a cost of performance. The optimal performance for the inspection task came with three discrete actions with $\controlmax=0.1~N$. In \figref{subfig:insp-ep-plot-dis_0.1_3}, it can be seen that this configuration also results in a much smoother trajectory, as the agent can make smaller adjustments to its trajectory due to the smaller $\controlmax$. Therefore, the optimal behavior can also be achieved using discrete actions for the inspection task. This also follows \figref{subfig:histogram-w}, where the actions most commonly used are zero and $\pm \controlmax$.

\begin{figure*}[t]
\centering
\subfigure[Continuous actions with $\controlmax=1.0~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/inspection/con_1.0.png}\label{subfig:insp-ep-plot-con_1.0}}\qquad
\subfigure[3 discrete actions with $\controlmax=1.0~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/inspection/dis_1.0_3.png}\label{subfig:insp-ep-plot-dis_1.0_3}}\qquad
\subfigure[101 discrete actions with $\controlmax=1.0~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/inspection/dis_1.0_101.png}\label{subfig:insp-ep-plot-dis_1.0_101}}
\subfigure[3 discrete actions with $\controlmax=0.1~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/inspection/dis_0.1_3.png}\label{subfig:insp-ep-plot-dis_0.1_3}}
\caption{Example episodes for policies trained in the inspection environment. The trajectory changes from light to dark as time progresses. Blue, red, and green lines represent the $x$, $y$, and $z$ components respectively.}
\label{fig:inspection_ep_plots_1}
\end{figure*}

For the docking task, ideally the agent will slow down and approach the chief along a smooth trajectory. \figref{fig:docking_ep_plots_1} shows example trajectories of trained agents in the docking task, where similar results to the inspection task can be seen. Continuous actions allow for the smoothest trajectory, three discrete actions with $\controlmax=1.0~N$ is the least smooth trajectory, and 101 discrete actions or three discrete actions with $\controlmax=0.1~N$ allow for smoother trajectories while using discrete actions. However, there is still a considerable amount of ``chattering" for the control, where the agent frequently switches between multiple control values as it attempts to refine its trajectory.

To best balance continuous and discrete actions, we analyze the behavior shown in \figref{subfig:histogram-bell}, and attempt to provide action choices for the agent that mimic a bell curve. These experiments are the $1.0/0.1$ configuration and the $1.0/../0.001$ configuration. These configurations allow the agent to use actions with high magnitudes when they are far from the chief, but small magnitudes when they get closer to the chief. From \figref{subfig:delta-v-0.1-dock} and \figref{fig:dock-reward-int-est}, it can be seen that the $1.0/../0.001$ configuration achieves much lower $\deltav$ than the $1.0/0.1$ configuration, with both having 100\% success. These configurations also achieve better reward and lower $\deltav$ than most discrete action experiments, but still do not perform as well as the agent trained with continuous actions. As shown in \figref{subfig:dock-ep-plot-1.0/0.1} and \figref{subfig:dock-ep-plot-1.0//0.001}, these configurations also do not have as smooth of trajectories as the agent with continuous actions, and there is still frequent chattering in the control. Therefore, despite attempting to balance discrete and continuous actions, the optimal behavior for the docking task is still achieved using continuous actions.


\begin{figure*}[t]
\centering
\subfigure[Continuous actions with $\controlmax=1.0~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/docking/con_1.0.png}}\qquad
\subfigure[3 discrete actions with $\controlmax=1.0~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/docking/dis_1.0_3.png}}\qquad
\subfigure[101 discrete actions with $\controlmax=1.0~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/docking/dis_1.0_101.png}}
\subfigure[3 discrete actions with $\controlmax=0.1~N$.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/docking/dis_0.1_3.png}}
\subfigure[5 discrete actions: $1.0/0.1$ configuration.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/docking/dis_1.0_0.1.png}\label{subfig:dock-ep-plot-1.0/0.1}}
\subfigure[9 discrete actions: $1.0/../0.001$ configuration.]{\includegraphics[width=0.48\linewidth]{figures/episode_plots/docking/dis_1.0_0.1_0.01.png}\label{subfig:dock-ep-plot-1.0//0.001}}
\caption{Example episodes for policies trained in the docking environment. For the trajectories, the chief's position is represented by a black star, and the deputy's initial position is represented by a red star. For the distance dependent speed limit, safe regions are shaded green and unsafe regions are shaded red.}
\label{fig:docking_ep_plots_1}
\end{figure*}

